AWESOME: Empowering Scalable Data Science on Social Media Data with an Optimized Tri-Store Data System

Modern data science applications increasingly use heterogeneous data sources and analytics. This has led to growing interest in polystore systems, especially analytical polystores. In this work, we focus on emerging multi-data model analytics workloads over social media data that fluidly straddle relational, graph, and text analytics. Instead of a generic polystore, we build a "tri-store" system that is more aware of the underlying data models to better optimize execution to improve scalability and runtime efficiency. We name our system AWESOME (Analytics WorkbEnch for SOcial MEdia). It features a powerful domain-specific language named ADIL. ADIL builds on top of underlying query engines (e.g., SQL and Cypher) and features native data types for succinctly specifying cross-engine queries and NLP operations, as well as automatic in-memory and query optimizations. Using real-world tri-model analytical workloads and datasets, we empirically demonstrate the functionalities of AWESOME for scalable data science over social media data and evaluate its efficiency.

==> sections/bulky-assignment.tex <==
\section{Bulk Assignment Algorithm}
Given a list of segments list $\mathcal{S} = [LS_1, \cdots, LS_n]$ and a predecessor mapping for detached chain heads $DCM$,  this section introduces the Bulk assignment algorithm  to schedule operators efficiently. 

% LA is a list of triple, [(operator index, assigned core, amortized time)], DO is a list of tuples [dominant operator index , dominant amortized time]


% \todo{explain the whole structure, select segments as candidate segments list, in each of $p$ iteration, choose a proper operator to assign core; TO satisfy the two constraints in definition, detached chains needs to be handled properly when scheduling }
We give an overview of the scheduling algorithm presented in Algorithm \ref{algo:schedule}. It maintains an unfinished chain list $unfChain$ which includes all unassigned segments in  each chain.  A candidate segments list $candSegs$ is maintained which contains a list of segments that serve as candidates to  be processed during the current single assignment. Initially, $unfChain = \mathcal{S}$ and $candSegs$ contains  the first segment from each chain.  As long as there are still unassigned operators left (line 3), a  single batch assignment will be initiated. In each single round, there are at most $p$ iterations and  in  each iteration, an operator from $candSegs$ will  be assigned  to a specific  core. Iteration ends until all $p$ cores are assigned or an early stopping rule satisfies. In the following subsections, we will explain the single batch assignment algorithm shown in Algorithm \ref{algo:single} with focus on the three details: 1)  how to process detached chain heads 2)  the select criteria to assign a core in each iteration and 3) how to update $candSegs$ and $unfChain$ after a single assignment finishes to prepare for the next single assignment. 




\subsection{DCH processing rules (lines 17 - 23)}
From Definition \ref{def:greedyproblem}, there are two constraints: operator dependency and indivisibility. However, 
a detached chain is included in multiple chains and will be scheduled multiple times, which   against  indivisibility. Also, a detach chain head  has more than one predecessors, when assigning a core to a head, the predecessors need to be checked to make sure that the dependency constraint is not violated. We provide the following  rules for DC to decide if this can be safely executed or be discarded from this chain:
\begin{definition} [Execution rule for detached chain]
\noindent\textbf{Execution Rule:} This operator can be safely assigned if one of the two cases happens, 
\begin{itemize}
    \item if all the predecessors have been assigned in previous rounds batch assignments
    \item if one predecessor which the head has pipeline or stream input capability on has been  scheduled in this round and all other predecessors have been assigned in previous rounds. 
\end{itemize}


\noindent\textbf{Discard Rule:}  If none of the above cases  satisfies, then this head operator and all its  successor operators in this chain will be discarded. 
\end{definition}

With the execution and discard rules, every operator in  detached chain will be guaranteed to be scheduled and executed only once. 

\subsection{Greedy assignment in each iteration}
In each iteration of a single batch assignment, an operator will be selected out to assign the current core. This decision should be made depending on which operator can save more of total execution time with this  core.  The single batch assignment will be initialized as assigning  all the first operators a distinct core and $candSegs$ are updated accordingly (lines 3-6).  


Suppose at the $i_{th}$ iteration, the current single-batch assignment is $X^i = (L^i, M^i)$, and the  list of candidate segments with unassigned operators is $candSegs^i$, then  when assigning the $i_{th}$ core,  there are some candidate operators to consider: first operators in each segment from $candSegs^i$, denoted as a list $candOpes$, and one operator, denoted as $op_{X^i}^{dom}$, which dominates the execution time of the  current assignment, i.e., $X^i$.
% % an operator to a pipeline scheduling, we are interested in how much time it can overlap with the existing pipeline scheduling. Intuitively, the more it overlaps with, the higher priority should be given to assign cores to it. Let $op_{sk}$ be the first operator on the segment that has not been added to a pipeline, and $P$ denotes a pipeline scheduling for all operators in $S$ before $op_{sk}$ along with their assigned core numbers, i.e., $P = \{(op_{si}, n_i)| \forall i<k\}$, then we need to decide how to assign the next available core. There are only two operators needed to be considered: 

% the dominant operator in the existing pipeline $P$ that determines the total execution time of this pipeline, and the current first unassigned operator $op_{sk}$. 

We formally define  dominant operator  and dominant execution time of a single batch assignment  as the following:
\begin{definition} [Dominant Operator and Dominant Execution Unit Time]
Giving an assignment  $X = (L, M)$, by summing up matrix $M$ by rows, we can get a list $N$ where $N[i]$ is the number of cores assigned to operator $L[i]$. A  list of amortized unit execution times for $L^i$ are computed as  $AMT =\{d^{au}_{i}\} = \{D^u_[L[i]]/N[i]\}$, then $max(AMT)$ will be the  dominant execution time $d_X^{dom}$ for assignment $X$, and the operator with this amortized unit time is the dominant operator $op_X^{dom}$. 
\end{definition}


% \todo{should change this, there are three t ypes of segments, dual-pipeline-able and single pipeline-able. For dual-pipeline-able, after a pipeline finish, should not just parallel executed the rest, instead should consider form another pipeline from the end}
% Whether to assign the current core to a $op^{dom}_P$ or $op_{sk}$ will depend on which can save the most time. 


Given   the candidate operators $candOpes$ and dominant operator $op_{X^i}^{dom}$, the saved execution time by assigning the current core to each of them will be computed. We introduce how to compute it for normal operator from $candOpes$ and the dominant operator.
Denote the updated single batch assignment after this iteration as $X^{i+1}$, the saved execution time for an   unassigned operator $op$ is computed as,
$$(US[op] \times d^{dom}_{X^i}  + DP(op)) - US[op]\times d^{dom}_{X^{i+1}}$$, 
where $DP(op)$ is the time cost to execute $op$ in parallel after this round finishes executing: $DP(op) =  \frac{D^u[op] \times US[op]}{p}$, and $d^{dom}_{X^{i+1}} = \max(d^{dom}_P, D^u[op])$. 


Suppose that the dominant operator in $L$ is $L[i]$, the saved execution time for the dominant operator is computed as,
$$ US[d^{dom}_{X^i}]\times(d^{dom}_{X^i} - d^{dom}_{X^{i+1}})$$, 
where  $d^{dom}_{X^{i+1}} =  \max(\{D^u[L[1]]/N[1], \cdots, D^u[L[i]]/(N[i] + 1), \cdots \}) $.


The operators are sorted in order of maximum saved time to minimum saved time. The first operator which is a non-DCH or a safely executed DCH will be compared with the dominant operator to decide the final runner (Line ). Note that in one situation, this operator will not get the current core and this single batch assignment will stop early: assigning the runner operator all the rest of cores will not save time than parallel execution, which is formally formulated as, 
$$(US[op] \times d^{dom}_{X^i}  + DP(op)) - \frac{D^u[op] \times US[op]}{p'} < 0$$,
where $p'$ is the number of available cores left. 



% \begin{itemize}
%     \item Suppose the dominant operator is the $i_{th}$ operator: $op_{si}$, after assigning it one more core,  the updated pipeline scheduling $P' = \{(op_{s1}, n_1), \cdots, (op_{si}, n_i + 1) \cdots, (op_{s(k-1)}, n_{k-1)})$, then the
%     saved time is computed as: $m_s\times(d^{dom}_P - d^{dom}_{P'})$. $d^{dom}_P = d^u_{si}/n_i$, and $d^{dom}_{P'} = max(AMT') = max(\{d^{au}_{s1}, \cdots, d^u_{si}/(n_i + 1), \cdots \})$.
%     \item If the core is assigned to $op_{sk}$, then $P' = P \bigcup \{(op_{sk}, 1)\}$,
%     the saved time is defined as: $(m_s \times d^{dom}_P  + d^{dp}_{sk}) - m_s\times d^{dom}_{P'}$, where $d^{dp}_{sk}$ is the time cost to execute $op_{sk}$ in parallel after the pipeline finishes and computed as $d^{dp}_{sk} = \frac{d^u_{sk} \times m_s}{p}$, and $d^{dom}_{P'} = max(d^{dom}_P, d^u_{sk})$. If $d^u_{sk} < d^{dom}_P$, it means that executing this operator by adding it to the  pipeline will not increase any of total execution time.  
% \end{itemize}
% for dominant operator is computed as:






% If assigning the current core to the dominant operator saves more time, then we should assign  to it, otherwise, assign to the next unassigned operator.


% \subsection{Revisit of scheduling algorithm}
% In each round of single assignment, 

% Initially, 





% Then, for the rest of ...




% candidate segments are initially the first segments from all chains, except the detached chain heads, the segments are independent from each other.  When scheduling, the first operators from all candidate segments are all assigned one core  are removed from  segments. A check function will be called if  the first operator is a  DCH  and the detached chain will either be kept or discard in this chain. The dominant operator and dominant time are updated. 
% After assigning first operators, the rest of available cores are assigned. The saved time for new first operators from each segment is computed and these operators are sorted by their saved time from maximum to minimum. The sorted operators will be processed until  a candidate operator is detected: if the operator is not a DCH, it is a candidate operator; if  it is a DCH and it can be executed in this round, it is a candidate operator. Then the candidate operator's save time will be compared with that of the dominant operator to decide which operator should  this core be assigned to.  If the optimal saved time is non positive, then this round of assignment should be early stopped.


% After a single round, the candidate segments need to be updated for the next round. Only in two cases, a candidate segment needs to be updated:  if a segment is empty which means all operators in this segment have been assigned, then the next segment from the same chain will be picked up. If a segment is marked as a discard chain, it means that all the successor  operators  in the chain where the segment is from form a detached chain which should not be executed in this chain, thus this chain will be updated as empty in the list of unfinished chains  $unfChain$, and the candidate segment is updated as  empty.


\begin{algorithm}[!h]
\caption{\emph{Bulk\_Assignment}}\label{algo:schedule}
\SetKwFunction{ComputeSavedTimeForCandidate}{ComputeSavedTimeForCandidate}
\SetKwFunction{ComputeSavedTimeForDominant}{ComputeSavedTimeForDominant}
\SetKwFunction{SingleBatchAssignment}{SingleBatchAssignment}
\SetKwProg{Fn}{Function}{:}{}
\KwIn{$\mathcal{S}, DCM$, batch sizes of  chains $M$}
% operators in each chain has the same batch sizes 
\KwOut{A list of single batch assignments $\mathcal{X}$. }
\tcc{initialize}
$\mathcal{X} \gets []; unfChain \gets \mathcal{S}; chainNum \gets \mathcal{S}.size; allAssignedOpe \gets \{ \}$\;
$ candSegs \gets [unfChain[i][0] \text{ for } i \in [0, chainNum]$\;
\tcc{if there is an unfinished chain, starts a single batch assignment}
\While{$ \exists i \in [0, chainNum): unfChain[i].size > 0 $}{
    % for each head of a chain, assign a core to the first operator of the chain as long as it is not a DCH.
    % if there is an unfinished chain, start a new batch assignment.
    % in each single-batch assignment, the candidate segments are the first segments from each chain. 

    $X, candSegs, discardChain \gets $ \SingleBatchAssignment $(candSegs, allAssignedOpe, D^u, US)$\;
   
}
$ allAssignedOpe.addAll(X.L) $\;
\tcc{Create candidate segments for the next single batch assignment}
% \tcc{when  a segment in the candidate segments list  finishes in one round, then remove it add the next segment in the chain to the candidate list, otherwise, keep it  }

\tcc{Discard some detached  chains to make sure they will only be  executed in one  chain}
\For {$ i \in discardChain $} {$unfChain[i], candSegs \gets [], []$}
\For{$i \in [0,  chainNum)$}{
    \tcc{for a segment which has finished assignment  in this batch, remove it from its chain }
    \If {$candSegs[i].size == 0$}{
        $unfChain[i].poll()$\;
        \lIf{$unfChain.size > 0 $}{$canSegs[i] \gets unfChain[i][0]$}
    }
    
}
\end{algorithm}



\begin{algorithm}[!h]
\caption{\emph{Single\_Batch\_Assignment}}\label{algo:single}
\SetKwFunction{SavedTimeForUnassign}{SavedTimeForUnassign}
\SetKwFunction{SavedTimeForDominant}{SavedTimeForDominant}
\SetKwFunction{SingleCoreAssignment}{SingleCoreAssignment}
\SetKwFunction{UpdateDominant}{UpdateDominant}
\SetKwFunction{EarlyStop}{EarlyStop}
\SetKwProg{Fn}{Function}{:}{}
\KwIn{A candidate segments list $candSegs$, assigned operators in previous rounds $ allAssignedOpe $, unit execution time $D^u$, execution unit sizes $US$ }
% operators in each chain has the same batch sizes 
\KwOut{A single batch assignment $X$, an updated $candSegs$, a discard list $discardChain$}
$L \gets []; M \gets []; AMT \gets [];  core \gets 0$\;
$discardChain \gets {}; chainNum \gets candSegs.size$\;
        % \tcc{initialize single batch assignment as assinging onefirst operators}
\For{ $ i \in [0, chainNum)$ } {
    $op \gets candSegs[i].poll(); L.add(op); core++$\;
        % % \If {$ !DCM.contains(op) $}{
        % $  candSegs[i].poll(); core ++$\;
    $ vec \gets zeros(1, p); vec[core] \gets 1; M.add(vec)$\;
    $ AMT.add(D^u[op]) $\;
        % \tcc{update local assignment schedule: assign $op$ one core }
        % $LAS[i].schedule(op, 1)$
}
    % should have AMT list for all assigned operators to compute the saved time 
\tcc{get dominant operator index and dominant amortize time}
$domOpe, domTime = AMT.argmax, \max(AMT)$\;

\For{$ c = core; c <p; c++ $} {
    \tcc{compute saved time for first unassigned operators}
    $ ope \gets [$ \SavedTimeForUnassign $(candSegs[i][0], domTime, US, D^u) \text{ for } i \in [0, chainNum)]$\;
    $ sortedOpe \gets ope.sort(key=\_.savedtime)$\;

    % the single segment scheduling returns the local optimal operator and its saved time
    % \For{$i \in [0, candSegs.size)$}{
    %     $LOO.add($\SingleSegmentSchedule($candSegs[i], LA[i], $)\;
    % }
    $domSavedTime \gets -Inf$\;
    \If{$domOpe.para == DP$} {
    $domSavedTime \gets$ \SavedTimeForDominant$(domOpe, domTime, AMT)$\;
    }
    \tcc{ decide which operator to assign }
    \For{ $ op \in sortedOpe $ }{
        \lIf{ $ !DCM.contains(op) $ } { break }
        \Else {
            $ parents \gets DCM.get(op)$\;
            \lIf {$ \forall p \in parents: p \in allAssignedOpe $}  { break }
            \Else {   $ unfP \gets parents - allAssignedOpe $\;
                \If {$unfP.size == 1 \&\& unfP[0] \in L \&\& op.capOn(unfP[0]) == P||I $}{break}
            }
            % \tcc{discard the whole detached chain from $unfChain$ since it will not be executed in this chain}
            $ discardChain.add(op.chainIndex) $ \;
            }
    }
    \tcc{decide to assign to dominant one or unassigned operator or stop the batch assignment}
    \If {$domSavedTime > op.savedtime$} {
        $M[L.idx(op), core] \gets 1$\; }
    \Else {
        \If {\EarlyStop$(op, US, domTime, D^u)$} {break}
        \Else {$L.add(op);vec \gets zeros(1, p); vec[core] \gets 1; M.add(vec)$}
    }
   \tcc{update dominant operator.}
   $AMT, domOpe, domTime \gets$ \UpdateDominant$(X, L)$\;
}
\Return $X, candSegs, discardChain$\;
\end{algorithm}


==> sections/problem-formulation.tex <==
\section{Preliminary}
We categorize AWESOME operators into four classes based on the pipeline capability:
\begin{itemize}
    \item Input Pipeline-able (I): The input of an operator can be processed batch by batch while the result can only be released when the whole execution finishes (e.g., aggregation operators). 
    \item Output Pipeline-able (O): The input of an operator is processed as a whole unit and can not be processed batch by batch, while it can be executed in an online manner where the results are released batch by batch before the whole execution finishes. (\todo{give examples like calculating shortest path and calculating node degrees})
    \item Blocking (B): The input of an operator is processed as a whole and the output can only be returned when execution finishes. 
    \item Pipeline-able (P): An operator is both input pipeline-able and output pipeline-able. 
\end{itemize}

A different way to classify an operator is based on its data parallelism capability:  
\begin{itemize}
    \item Data Parallel-able (DP): The input of an operator can be partitioned and the operator can be executed by executing each partition and unifying results;
    \item Serialized (S): An operator is not data parallel-able.
\end{itemize}


\subsection{Notations and Definitions}

\begin{table}
\caption{Notations used in definitions} \label{tab:simplenotation}
\centering
\begin{tabular}{l|p{0.3\textwidth}} 
\toprule
Symbol & Description \\
\midrule
$p$ & the number of processors \\\hline
$P$ & a set of processors $P = \{P_1, \cdots, P_p\}$\\\hline
$op$ & an operator \\\hline
$n$ & the number of operators \\\hline 
$OP$ & a set of operators $OP = \{OP_1, \cdots, OP_n\}$ \\\hline 
$G = \{OP, E\}$ & a physical plan DAG \\\bottomrule
\end{tabular}
\end{table}

We first present a set of definitions. Table \ref{tab:simplenotation} summarizes the notations used hereafter.
\begin{definition}[Operator]
An operator $op$ refers to a physical operator associated with two attributes: pipeline capability $op.pipe \in \{I, O, B, P\}$ and parallelism capability $op.para \in \{DP, S\}$. Table~\ref{tab:operatornotation} summarizes the common notations for operators.
\end{definition}

Note that, for an operator $op$ where $op.pipe = O, B$, it has to be serialize-able since the input can't be partitioned.  For $op$ where $op.pipe = I, P$, $op.para$ can be either $DP$ or $S$. (\todo{give example, write to DBMS should be serialized.}).



\begin{definition} [Physical Plan]
A physical plan is defined as a Directed Acyclic Graph (DAG) $G = \{OP, E\}$ where $OP$ is the set of operators and $E$ is the set of edges (i.e., connections between operators).
% connecting operators: $E = \{e | e.in = op_i, e.out=op_j \text{ where } op_i, op_j\in OP\}$.
\end{definition}


\begin{definition}[Execution Unit]
For an operator $op$, if $op.pipe = I$, the execution unit denotes an input data batch; if $op.pipe = O$, the execution unit denotes an output data batch; if $op.pipe = B, P$, the execution unit can denote either an input or output data batch.
\end{definition}

\begin{definition}[Task]
A task $t$ is defined as a tuple $(op, i)$ where $op$ is an operator, and $i$ is the $i$-th execution unit of $op$. 
Table~\ref{tab:tasknotation} summarizes notations for tasks.
\end{definition}


% We define notations for operators in Table \ref{tab:operatornotation}. Since tasks are the units of the scheduling problem, we also define some notations on tasks in Table \ref{tab:tasknotation}.

\begin{table}
\caption{Operators Notations} \label{tab:operatornotation}
\centering
\begin{tabular}{l|p{0.33\textwidth}} 
\toprule
Symbol & Description \\
\midrule
$D = \{d_i\}$ &  the total execution time (duration) of each operator $op_i \in OP$ \\ 
% \hline
% $D^0 = \{d^0_{i}\}$  & \begin{tabular}[c]{p{0.45\textwidth}}
% if $op_i.pipe = I$, $d^0_i$ is the execution time to finish $op_i$ after processing all execution units \\
% if $op_i.pipe = O$, $d^0_i$ is the execution time needed for $op_i$ to release the first execution unit \\
% if $op_i.pipe = P$, $d^0_i = 0$ \\
% if $op_i.pipe = B$, $d^0_i = 0$ \\
% \end{tabular}  \\ 
\hline
$D^u = \{d^u_{i}\}$  & $d^u_i$ is the execution  time of $op_i$ processing/releasing a single execution unit. If $op_i.pipe = B$, $d^u_i = d_i$. \\ 
\hline
$IS = \{is_i\}$ & $is_i$ is the number of input execution units of operators. If $op_i.pipe = O \text{ or } op_i.pipe = B$ , $is_i = 1$. \\\hline
$OS = \{os_i\}$ & $os_i$ is the number of output execution units of operators. If $op_i.pipe = I \text{ or } op_i.pipe = B$, $os_i = 1$.\\\hline
$US = \{us_i\}$ & the numbers of execution units of operators.  \\\hline
$OP^p \in \{0, 1\}^{|OP| \times p}$ & Operator assignment matrix. $OP^p_{i, j} = 1$ if $op_i$'s execution units are assigned to processor $j$. \\\bottomrule
% $OP_{i, j}$ & the $j_{th}$ operator on core $i$ \\\hline 
% $P_{op}$  & a set of cores that $op$ is assigned to. \\
% \hline
% $S = \{s_i\}$      & Execution start time of operators. \\\hline
% $S^u$ & $S^u_{i, j}$ is the execution start time of $op_i$'s $j_{th}$ unit. If $op_i.pipe = B, O$, then $j\in \{1\}$.\\
% \hline
% $E = \{e_i\}$      & Execution finish time of operators \\\hline
% $S^p \in \mathbb{R}^{|OP| \times p}$ & $S^p_{i, j}$ is the start time of $op_i$ on core $j$. $S^p_{i, j} = \infty, \text{ for } \forall i, j \text{ where } OP^p_{i, j} = 0$.\\
% \hline
% $E^p \in \mathbb{R}^{|OP| \times p}$ & $E^p_{i, j}$ is the end time of $op_i$ on core $j$. $E^p_{i, j} = 0, \text{ for } \forall i, j \text{ where } OP^p_{i, j} = 0$. \\ 
% \hline
\end{tabular}
\end{table}

\begin{table}
\caption{Task Notations} \label{tab:tasknotation}
\centering
\begin{tabular}{l|p{0.23\textwidth}} \toprule 
Symbol & Description \\
\midrule
% maximum number of units 
$N$ & the maximum number of units. $N = \max(US)$ \\\hline 
% task matrix 
$T = \{t_{i, j}\}, i\leq |OP|, j\leq N$ & Tasks matrix. $t_{i, j}$ is the task $t(op_i, j)$ \\\hline
% start time of each task, if no such unit, should be 0. 
$ST \in \mathbb{R} ^ {|OP|\times N} $ & Start time matrix. $st_{i, j}$ denotes the start time of task $t(op_i, j)$\\\hline
% execution time of each unit. If no such unit, should be 0 
$DT \in \mathbb{R} ^{|OP|\times N}$ & Execution time matrix. $dt_{i, j}$ denotes the execution time of task $t(op_i, j)$\\\hline
$ET \in \mathbb{R} ^{|OP|\times N}$ & End time matrix.\\\hline   
% distribution matrix: each unit needs to be executed only once 
$A \in \{0, 1\} ^ {|OP| \times N \times p}$ & Assignment Matrix. $A_{i, j, k} = 1$ iff $op_i$'s $j_{th}$ unit is assigned to processor $k$. \\\hline  
% task dependency matrix: based on operator dependency and also parallel capability 
$TD \in \{0, 1\} ^{(|OP| \times N)\times (|OP| \times N)}$ & Task dependency matrix. $td_{(i, j), (k, h)} = 1$ iff $t_{k, h}$ depends on $t_{i, j}$.  \\\bottomrule  

% $OP_{i, j}$ & the $j_{th}$ operator on core $i$ \\\hline 
% $P_{op}$  & a set of cores that $op$ is assigned to. \\
% \hline
% $S = \{s_i\}$      & Execution start time of operators. \\\hline
% $S^u$ & $S^u_{i, j}$ is the execution start time of $op_i$'s $j_{th}$ unit. If $op_i.pipe = B, O$, then $j\in \{1\}$.\\
% \hline
% $E = \{e_i\}$      & Execution finish time of operators \\\hline
% $S^p \in \mathbb{R}^{|OP| \times p}$ & $S^p_{i, j}$ is the start time of $op_i$ on core $j$. $S^p_{i, j} = \infty, \text{ for } \forall i, j \text{ where } OP^p_{i, j} = 0$.\\
% \hline
% $E^p \in \mathbb{R}^{|OP| \times p}$ & $E^p_{i, j}$ is the end time of $op_i$ on core $j$. $E^p_{i, j} = 0, \text{ for } \forall i, j \text{ where } OP^p_{i, j} = 0$. \\ 
% \hline
\end{tabular}
\end{table}







% Suppose that there are a set of $n$ operators: $\{OP\} = op_1, op_2, \cdots, op_n$, and $op_{i+1}$ depends on $op_{i}$.  The first operator is the first category and the others are pipeline-able and parallel-able operators. Suppose that the execution time of $op_1$ releasing one batch of data is  $t_1$, the execution time of $op_i, i>1$ processing one batch is $t_i$, and the number of available cores of the OS is $p$, the problem is to find a scheduling strategy  to minimize the total make-span of executing all operators in set $\{OP\}$.

\subsection{Physical Plan DAG to Tasks Set}
Since the input of the scheduling problem is a physical plan DAG, while the tasks are the units to be scheduled, the DAG $G$ should be properly transferred to a tasks set $T$ while maintains all the properties of operators. 


Given a DAG $G$,  then the task matrix $T$, the  execution time matrix $ET$ and task dependency matrix $TD$ should be created from it:

\noindent\textbf{Task matrix $T$:} $T$ has the dimension $|OP| \times N$ where $N = max(US)$. 


\noindent\textbf{Execution Time Matrix $ET$:} 
$$ dt_{i, j}=\left\{
\begin{aligned}
d^u_i  & \text{  ,  if } j\leq is_i \\
0 & \text{  ,  otherwise.}\\
\end{aligned}
\right.
$$


\noindent\textbf{Task Dependency Matrix $TD$:} There are two types of tasks dependency: 
\begin{itemize}[leftmargin=*]
    \item Operators dependency: if $op_{i'}$ depends on $op_{i}$, $td_{(i, j), (i', j)} = 1$;  
    \item Self dependency: if $op_i.para = S$, then  $td_{(i, j), (i, j')} = 1, \forall j' > j$.  
\end{itemize}


% \todo{the problem definition should treat tasks as schedule units and consider tasks dependency based on its operator, and if the operator has a S parallel capability, then each unit depends on its own last unit. If pipe is O, B, then each one depends on the last one of the last operator (needs to wait for the last unit of last operator finishes. If I, P, depends on the last operators' the same unit). Should have a task dependency matrix}




\subsection{Problem Formulation}
Given a physical plan DAG $G = \{OP, E\}$, a task matrix $T$, execution time matrix $ET$, and task dependency matrix $TD$ can be created from it. The problem is to distribute tasks in $T$ to $p$ processors to minimize the total make-span, i.e., to solve assignment matrix $A$ and start time matrix $ST$ to minimize the maximum of task end time $max(ET)$:
\begin{equation}
\begin{aligned}
\min_{A,\, ST} \quad & \max(ET)\\
\textrm{s.t.} \quad & \textcircled{1} st_{i, j} \geq td_{(i', j'), (i, j)}(st_{i', j'} + dt_{i', j'}), \\
  &\quad\quad\quad \forall (i', j'), (i, j) \in [1, \cdots, |OP|]\times [1, \cdots, N];\\
  & \textcircled{2} et_{i, j} = st_{i, j} + dt_{i, j},  \\
  & \quad\quad\quad \forall (i, j) \in [1, \cdots, |OP|]\times [1, \cdots, N];\\
   & \textcircled{3} \sum_{k'=1}^p A_i, j, k' = 1,\\
   & \quad\quad\quad \forall (i, j) \in [1, \cdots, |OP|]\times [1, \cdots, N];\\
  & \textcircled{4} (st_{i, j} - et_{i', j'})(et_{i, j} - st_{i', j'}) \geq 0, \\
  & \quad\quad\quad \forall k\in [1, \cdots, p], \forall (i, j), (i', j') \in [(i_x, j_x)|A_{i_x, j_x, k} = 1].
\end{aligned}
\end{equation}

The constraints are:
\begin{enumerate}[label=\protect\textcircled{\arabic*}, leftmargin=*]
    % \item Processor consistency: for a core $i$, it needs to wait for the current  operator to globally finish  before executing the next one on this core: $SP_{OP_{i, j+1}} \geq E_{OP_{i, j}}$. \todo{is this correct?}
    \item \emph{Task dependency:} A task needs to be executed after its depend-on tasks finish. 
    \item \emph{Non-preemptive execution:} A processor finishes each task non-preemptively. 
    \item \emph{Indivisibility:} A task needs to be assigned to exactly one processor. 
    \item \emph{Processor exclusive access:} A processor can only execute one task at a time. The execution times of two tasks on the same processor can not overlap. 
    
    % \item Processor availability: when assigning an operator to cores, these cores need to be available: 
    % for any core $i$, we have $S_{OP_{i, j+1} > E_{OP_{i, j}}}$ 
    % \item One time assignment at start time: When assigning an operator, we should only consider the available cores at the time when the operator starts, and we should not add more cores even if  there are more cores available in the middle of execution. \todo{is this correct?}
\end{enumerate}
\subsection{Proof of NP hardness} 




==> sections/scheduling-algorithm.tex <==
\section{Operator-Level Greedy Schedule}
In this section, we provide a greedy strategy which schedules at operators level instead of tasks level. \todo{maybe provide some intuition about using operator-level schedule}

% We first provide some assumptions for the operator-level scheduling:
% \begin{itemize}[leftmargin=*]
% \item The operators are assigned to cores in multiple rounds until all operators have been assigned. Each round is called a single assignment where some operators will be chosen to be assigned to $p$ cores. During a single assignment, when one core finishes its task in the middle, it will be idle until this single  assignment finishes.
% \item When an operator is assigned to multiple cores, these cores should start and end at the same time. \todo{maybe this is unnecessary}
% \end{itemize}

\subsection{Problem Formulation}
We begin with the unit of operator-level schedule called \emph{Single Batch Assignment}. 

\begin{definition}[Single Batch Assignment]
A single batch assignment is defined as $X = (L, M)$ where $L = \{op_1, \cdots, op_l\}\subseteq OP$ ($l\leq p$) and $M$ is a matrix of dimension $p\times l$. Specifically, $M[i, j] = 1$ if worker $i$ executes operator $j$; otherwise, $M[i, j] = 0$. 
\end{definition}

In a single batch assignment, a worker can only process exactly one operator, i.e., $\sum_{j=1}^l M[i, j] = 1$ for $\forall i=1, \cdots, p$; however, an operator can be assigned to multiple cores. 

\begin{definition}[Operator-Level Schedule Problem] \label{def:greedyproblem}
% for operators with dependencies, when an operator is assigned, the dependent-on operator has already be assigned. each tuple has an order-ed list which is the operators be assigned in this batch with assignment orders. Dependency: when an operator is assigned, all its dependent-on operators have been assigned. 
The operator-level scheduling problem is to find a list of single batch assignments: $\mathcal{X} = \{X_1, \cdots, X_m\}$, named as Bulk Assignment, to minimize the makespan of the execution subjecting to the following constraints:
% $C(\mathcal{X})$, where $C(\cdot)$ is a function that calculates the makespan of an assignment, 
\begin{itemize}[leftmargin=*]
    \item \textbf{Operator Dependency:} when an operator is assigned, the predecessor operators should  already be assigned. 
    % Let $op_{ij}$ be the $j$-th operator in $L_i$ and $S$ be its corresponding dependency operator set. Then, for $\forall op' \in S$, we have  $op' \in L_i[:j-1] ||(\exists k\in [1, i) op'\in L_{k})$.  
    \item \textbf{Operator Indivisibility:} an operator should be assigned in exactly one single batch assignment: $L_i \cap L_j = \emptyset, \bigcup L_i = OP$. 
\end{itemize}
\end{definition}





% i.e.,  when an operator is assigned to a core, the core will execute this operator until the operator finishes. Even though there can be idle time, it will not execute other operators in the middle. 

% there are unassigned sub-chains, which may be detached to one of its parent chains.



\subsection{Chain and Segment Partition}
To satisfy the two constraints in Definition \ref{def:greedyproblem}, the operators in DAG $G$ need to be organized well. We provide chain and segment definitions in this section for the ease of scheduling. 
We first define a chain and  a detached chain as follows:
% \todo{when segment a chain, a->c, b->c, if c has pipeline/I capability on one of a, b, then should add c to that one; if c block/O or pipeline on both, cut both}

% should change the definition of chain which should include detached chain 

\begin{definition}[Chain]
Given a DAG $G = \{OP, E\}$, a chain is the longest list of operators satisfying that $C = [op^c_{1}, \cdots, op^c_{n}]\subseteq OP$ where $(op^c_{i}, op^c_{i+1}) \in E, \forall i\in[1, n)$ and $(op^c_{i}, op^c_{j}) \notin E \forall j\neq i+1$. 
% For any  operator in the chain except the last one, it has exactly one successor in the DAG which is its next operator in chain.
\end{definition}


\begin{definition}[Detached Chain]
Given a DAG $G = \{OP, E\}$ and a  chain $C = [op^c_1, \cdots, op^c_n]$, if $\exists op^c_i\in C: \exists op' \in OP: op' \notin C \&\&  (op', op^c_i) \in E $, then the sub-list $C' = [op^c_i, \cdots, op^c_n]$ is a detached chain, and $op^c_i$ is a detached chain head.
\end{definition}

Fig.~\ref{fig:seg} illustrates chains and detached chains. The physical DAG consists of operators denoted by circles and data flow dependencies  denoted by  the  black arrows. Each chain is denoted by operators and arrows with the same color other than black   connecting them. There are four chains in this DAG. A  detached chain is denoted by operators connecting by arrows with more than one non-black colors. For example, $[op_4, op_6, op_8, \cdots]$ forms a detached chain which is included by $c_1$ and $c_2$, and $op_4$ is the detached chain  head. 
Note that a  detached chain can be nested, i.e., a detached chain may contain another detached chain. For example, $[op_4, op_6, op_8, \cdots ]$ contains another detached chain starting from $op_6$ which are included by three chains. 


Given a chain $C = [op_1, \cdots, op_n]$, the chain will be partitioned to segments  where each operator belongs to exactly one segment. 

\begin{definition} [Segment]
A segment is a list  of operators. There are two types of segments:


\noindent \textit{Single-operator Segment:} For an operator $op$, $op$ itself is a single segment if it can not join or form a pipeline with its predecessors or  successors, i.e.,  any of the following conditions satisfies, 
\begin{itemize}
    \item  $op.pipe = B$.
    \item its predecessor's pipeline capability is $I$ or $B$, and its successor's pipeline capability is $O$ or $B$.
\end{itemize}


\noindent\textit{Schedule-able Segment:} It is a sub-chain $S = [op_i, op_{i+1}, \cdots, op_{j}]$ which satisfies:
\begin{itemize}
    \item Pipeline-able: $op_i.pipe = P||O, op_{j}.pipe = P||I, op_{k}.pipe=P \text{ for } \forall j\in (i, j).$
    \item Longest: $op_{i-1}$, and $op_{j+1}$ can not join this pipeline.
\end{itemize}
\end{definition}
% Note that hereafter segments mean the schedule-able segments. 

\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{figures/logical-plan-branch.pdf}
    \caption{Illustration of Chains and Detached Chains}
    \label{fig:seg}
\end{figure}

 
% Firstly, every  branch will be cut out to chains and the dependencies information is kept. As Fig.\ref{fig:seg} illustrates, the sub-DAG is separated to four chains and we have $C_1\to C_3$, $C_2\to C_3$ and $C_2\to C_4$. Then each chain is separated to a set of segments by the following rules: \todo{explain detail}. In Fig.\ref{fig:seg}, we have $C_1: \{s_{11}, s_{12}\}, C_2:\{s_{21}\}, C_3:\{s_{31}\}, C_4:\{s_{41}\}$.

% operator to cores that are available at the start time of this operator. 
% We first define available processors as follows,
% \begin{definition}[Available processor]
% A processor $i$ is available only when the current operator $op$ assigned to it  has been finished on all cores. 
% \end{definition}
% Note that when a processor finishes the execution units of $op$ that are assigned to it does not necessarily mean this core is available. It needs to wait for $op$ to finish to be available. 


% Based on the definition of available cores, we provide two assumptions for the coarse greedy algorithm, 
% \begin{itemize}
%     \item Processor availability: when assigning an operator to cores, it can only be assigned to  available cores.
%     \item One time assignment at start time: Each operator is only assigned once and will not add more cores to execute it even if  there are more cores available in the middle of execution.
% \end{itemize}

% We have the following equations:\\
% If $op_i.pipe = I$, then $t_i = t_i^0 + t_i^u * IS_i$, else $t_i = t_i^0 + t_i^u * OS_i$. \\
% $OS_i = IS_{i+1}$ (for chain only, for branches, it should depend on which parent operator is the outer loop)\\
% $S_i = \min\{S_{op_i, j}\} \text{ where } j \in P_{op}$\\
% $E_i = \max\{E_{op_i, j}\} \text{ where } j \in P_{op}$\\



%% calculate overlap time for each core to each operator.
\subsection{Scheduling Algorithm Overview}
Algorithm~\ref{algo:greedy} presents the framework to solve the operator-level schedule problem as defined in Definition~\ref{def:greedyproblem}. Given a physical plan DAG $G=\{OP, E\}$, we first partition $G$ to chains and some chains may have detached chains,  then each chain will be  partitioned to a set of segments. Then the Bulk Assignment   algorithm will be called to get the assignment result $\mathcal{X}$.

\begin{algorithm}[h]
\caption{\emph{Greedy\_Scheduling\_Framework}}\label{algo:greedy}
\KwIn{A physical plan DAG $G = \{OP, E\}$, where each operator $op \in OP$ has its pipeline capability: $op.pipe \in \{B, I, O, P\}$, parallelism capability $op.para \in \{DP, S\}$, and an operator id $op.id$}
\KwOut{A list of single batch assignments $\mathcal{X}$}
\SetKwFunction{PartitionChains}{PartitionChains}
\SetKwFunction{PartitionSegments}{PartitionSegments}
\SetKwFunction{BulkAssignment}{BulkAssignment}
\SetKwProg{Fn}{Function}{:}{}
\tcc{Get all chains and detached chain heads with their predecessors.}
$\mathcal{C}, DCM \gets $\PartitionChains($G$) \;
$\mathcal{S} \gets$ \PartitionSegments($ \mathcal{C} $) \;
$L \gets$ \BulkAssignment($\mathcal{S}, DCM$)\;
\end{algorithm}

\todo{maybe delete these two pseudocode? }
We provide the algorithms of partitioning DAG to chains and chain to segments in Algorithm~\ref{algo:chains} and Algorithm~\ref{algo:segs}. 

\begin{algorithm}[h]
\caption{\emph{Partition\_Chains}}\label{algo:chains}
\KwIn{$G = \{OP, E\}$}
\KwOut{A list of chains $\mathcal{C}$, a mapping from some operators to their predecessors $DCM$. }
$assignedOpe \gets \{\}; C\gets []; orderedOP \gets OP.sort(key=id)$\;
% $C \gets \{\}, assignedOpe \gets \{\}, detachHeadOpe \gets \{\}$\;
% $chainNum \gets 1, detachChainNum \gets 1$\;
% $MoC \gets \{\}, DoC \gets \{\}, MoDC \gets \{\}, DoDC \gets \{\}$\;
\For{$op \in orderedOP$}{
\tcc{For  an operator which has not  been assigned, since the operators are processed by orders,  it does not have any predecessor, thus it can form a chain.}
    \lIf {$op \in assignedOpe$}{continue;}
    $C.add(op), dHead \gets false$\;
    \tcc{add successors to chain}
    \While{$G.child(op).size == 1$}{
        $child \gets G.child(op)$\;
        \If{$G.parent(child).size> 1 \&\& !dHead $}{
%            \tcc{if the detached head operator is a blocking }
            \tcc{for detached head operator, add its predecessor operator to map }
            $ dHead \gets true; DCM[child].add(op))$\;
        }
         $op \gets child, C.add(op)$\;
        % \tcc{for branches like op->child, op'->child}
        % \Else{
        %     $sibling \gets G.predecessor(child)$\;
        %     \tcc{if $child$ is already in another chain, skip}
        %     \If{$child \in assignedOpe$}{break;}
        %     \tcc{if $child$ blocks on input or blocks on this current operator, then cut them directly.}
        %     \ElseIf{$(child.pipe == B || O) || (op \notin child.capOn)$}
        %     {break}
        %     \tcc{if $child$ has not been marked as a detached chain and its other predecessors have been processed, then it will be assigned to current chain.}
        %     \ElseIf{$child \notin detachHeadOpe \&\& \max([i.id for i \in sibling]) == op.id$} 
        %     {$op \gets child, C.add(op)$; }
        %     \tcc{if $child$ can join pipeline with the current chain and not the other chains, then assign it to current chain}
        %     \ElseIf{$child.capOn == \{op\}$}{$op \gets child, C.add(op)$; }
        %     \tcc{if $child$ can join with multiple pipelines, then mark it as the beginning of a  detached chain, and add map from it to the current chain.}
        %     \Else {
        %         \lIf{$child \in detachHeadOpe$} {$ DoDC[child].add(chainNum) $}
        %         \Else{$detachHeadOpe.put(child, )$}
        %         break\;}
            % there are two cases, maybe already been assigned as a detached chain, then just add to the set. 
        
            % \break 
            % \If{$(child.pipe == I \text{ or } P) \&\& (child.capOn = op)$}{
            %     $op = child$\;
            %     $C.add(op)$\;
            % }
            % \Else{break;} 
    }
    \tcc{add chain to chain list and initialize chain for the next round}
    $\mathcal{C}.add(C); C \gets []$\;
}
\end{algorithm}


\begin{algorithm}[h]
\caption{\emph{Partition\_Segments}}\label{algo:segs}
\KwIn{A list of chains $\mathcal{C}$}
\KwOut{A list of segments lists $\mathcal{S}$ where $\mathcal{S} = [LS_1, \cdots ]$ and $LS_i$ is a list of segments.}
$\mathcal{S} \gets []$\;
\For{$ C \in \mathcal{C}$}
{
    $LS \gets []; S\gets []$\;
    $start, end \gets 0$\;
    \For{$start \in [0, |C|)$}{
        \lIf{$start < end$}{continue}
        $crtOpe \gets C[start]; S.add(crtOpe)$\;
        \tcc{a single-operator segment which can't start a pipeline}
        \lIf { $crtOpe.pipe == B||I$ } { $end \gets start+1$ }
        \tcc{start  a pipeline}
        \Else{
            $end = start+1$\;
            \tcc{add to pipeline}
            \While { $C[end].pipe == P$ } {
                $S.add(C[end]), end++$\;}
            \If { $ C[end].pipe == I $ }{ $ S.add(C[end]); end++ $ }
        }
        \tcc{add current segment to segment list }
        $ LS.add(S); S\gets [] $
    }
    $\mathcal{S}.add(LS); LS \gets []$
}
\end{algorithm}



We first cut DAG to chains  as shown in Algorithm \ref{algo:chains} and a detached chain  can be included in multiple chains. The detached chain heads and their predecessors are detected by Lines 7-8. 
 Then each chain will be partitioned  to   segments as Algorithm \ref{algo:segs} shows: line 9  detects the single-operator segments, and lines 10 - 15 finds the longest pipeline.  The output of Algorithm \ref{algo:segs} is a list of segment lists: $\mathcal{S} = [LS_1, \cdots] $ where $LS_i$ is a list of segments. The BulkAssignment algorithm will be introduced in the next section.  
 
 






















% As previously stated, A DAG $G$ is partitioned to chains with dependencies, and each chain is then partitioned to a set of segments, and the chains dependencies will be propagated the dependencies among segments sets. For example, in Fig.\ref{fig:seg}, segments set $\{s_{31}\}$ depends on segments set $\{s_{11}, s_{12}\}$. 


% dominate one, then : m_i * d^{au}_{ij} - m_i * max(d^u_i*n_i/(n+1),  ).






% When partitioning $G$ to chains, we keep the dependencies among chains, then we have dependencies among segments sets. All independent segments sets without un-scheduled depend-on segments will be scheduled at the same time.   For example, in Fig.~\ref{fig:seg}, since $C_1$ and $C_2$ are not dependent, $\{s_{11}, s_{12}\}, \{s_{21}\}$ will be scheduled at the same time. 


% Assume that there are $n$ independent segments sets, each single segment maintains its local pipeline scheduling. Firstly, each first operator in each set will be assigned a core and each local pipeline scheduling is initialized with the first operator with one core. 
% Then, we assign the rest of available cores one by one. For each segment, the previous single-segment scheduling will be called to get the local to-be-assigned operator and saved execution time: $\{(op^*_1, st_1), \cdots, (op^*_n, st_n)\}$. Then the local operator with the maximum saved time will be chosen, and this local pipeline scheduling will be updated accordingly.  After all cores are assigned, the rest operators will be executed in parallel using all cores one by one.  The worst time complexity of this multi-segment scheduling is $O(p \times (\log(|OP|) +  \log(|OP|))))$.
% The overlap time should depend on how many cores that are assigned to an operator $op$, so  we define overlap time on $(P, op, n)$   where $P$ is a pipeline scheduling, $n$ is the number of cores assigned to $op$ as the following,  
% \begin{definition}[Overlap Time on $(P, op, n)$]
% Let $P$ denotes a set of operators along with their assigned cores number that in an existing  pipeline scheduling, i.e., $P = \{(op', n')\}$, and let $op$ denote the succeeding operator where $op.pipe = I \text{ or } P$, then the overlap time on $(op, n)$ is defined as, 
% $$d^{(P, op, n)}_{overlap} = d^P_{pipe} + d^{op}_{dp} - d^{P\cup\{(op,  n)\}}_{pipe}$$,
% where $d^{A}_{pipe}$ denotes the total execution time of a pipeline scheduling $A$, $d^{\cdot}_{dp}$ denotes the execution time of executing an operator in parallel using all cores (if it is serialized operator, then it denotes the serialized execution time).
% \end{definition}



% In the following, we present how to calculate $d^{P, op, n}$. Suppose that there exists a pipeline scheduling $P = \{(op_1, n_1), \cdots, (op_{k}, n_{k})\}$, and suppose that the dominate operator in this pipeline is $op_{dom}$ and  the total execution time depends on its amortized unit time: $d^u_{k}$ (we will explain later how $d^u_{k}$ is calculated).  




% Assume that  the size of $\{OP\}$ is 2. If  $op_1.pipe = O \text{ or } (op_1.pipe = P \text{ and } op_1.para = S)$, then $op_1$ can't take the advantage of data parallelism, and should consider executing the following operators in pipeline with it to decrease the total execution time. Suppose that $op_2.pipe = P$, then there are two cases: If $op_2.para = S$, then $op_2$ should be added to the pipeline with $op_1$; else, $op_2.para = DP$,
% then it is easy to prove the following:
% \begin{itemize}
%     \item if $d^u_2 < \frac{d^u_1}{1-\frac{1}{p}}$, add $op_2$ to pipeline and assign it one thread. 
%     \item if $\frac{(k-1)d^u_1}{1-\frac{k-1}{p}} < d^u_2 < \frac{kd^u_1}{1-\frac{k}{p}}$, add $op_2$ to pipeline and assign it $k$ threads if $k<p$, else assign $p-1$ threads.  
%     \item if $d^u_2 > p(p-1) d^u_1$, then should execute $op_2$ in parallel after $op_1$ finishes. 
% \end{itemize} 


% Assume that $|OP| > 2$, for $op_2$, schedule it as stated in the above, then when scheduling $op_3$, there are three cases depending on $op_2$'s scheduling. Let $d$ denote the time that $op_3$ should compare with, $d = d^u_1$ initially, and after deciding the  scheduling of $op_2$, $d$ should be updated: If $op_2.para = S$, then $d = \max(d^u_1, d^u_2)$; else, it should be updated as the following, 
% \begin{itemize}
%     \item if  $d^u_2 > p(p-1) d^u_1$, then $d=0$ which means the following operators will not join the pipeline. 
%     \item if $d^u_1 > \frac{d^u_2}{n}$ where $n$ is the number of threads that was assigned to $op_2$, $d = d^u_1$.
%     \item if $d^u_1 \leq \frac{d^u_2}{n}$, then $d = \frac{d^u_2}{n}$. 
% \end{itemize}

% After updating $d$, use the same strategy to schedule $op_3$ as used when deciding $op_2$ by replacing $d_1$ with $d$. Repeat the steps when  one of the four cases happens: 1. $op_i.pipe = I$, then add $op_i$ to pipeline and then finishes  this pipeline (the later operators will not be added to it). It is easy to prove that $op_i$ should always be added to pipeline as long as there is an available core 2. all cores all assigned when deciding $op_i$. 3. When the scheduling strategy decides not to add the current   operator  to the pipeline, then the following operators will not join, the pipeline is closed. 

% \subsection{Branch}
% We first consider a branch with three operators: let $op^b_l$, $op^b_r$ denote the two direct predecessors of a branch and $op^j$ denote the successor operator of the branch. There are three cases and the scheduling for each case is different.

% \subsubsection{$op^j$ is not able to join }
% For the first case, if $op^j$ can not join any pipeline, i.e., $op^j.pipe = B \text{ or } op^j.pipe = I$, then 
%   $op^b_1.pipe=I, B$, and $op^b_2.pipe=I, B$. 




% \subsection{Multi-Segments Scheduling}
% % needs to consider how to balance the rates of the two incoming segments for branch with joint node being Pipeline-able. Maybe just cut the branches.

% % it actually also considers task parallelism

% The physical plan DAG $G$ will be partitioned to a segments set with dependencies among segments. We iterate each operator in order and partition it based on the  following rules:

% how to locate the beginning and end of a chain 
%% 0. cut: all branches will be cut, all operators with pipe = B will be cut to chains with dependencies, each operator with block capability. It will output chains with dependencies; 1. after cut, each will be a chain, then apply a simple algorithm to partition chain to segments with dependencies (the algorithm would include assigning true execution mode and then decide beginning and end) and besides segments dependencies, segments also maintain the chain dependencies. 
%%% for partitioning, first decide execution mode: there is only one parent and one child, so it is trivial: for the current operator, if the parent's execution mode is P or O, then .....; then decide segments' start and end: ;
% at each stage,choose an operator from any segment who does not have unsolved dependency, when assigning a core, it can be the current operator if it can be executed in parallel, also, it can be the next one. calculate saved time and update d for the selected segment. 




% \begin{itemize}
%     \item if chain, then 
%     \item if intersection, cut it,
%     \item 
% \end{itemize}










  
  

